Sound-Guided Semantic Video Generation

The recent success in StyleGAN demonstrates that pre-trained StyleGAN latent space is useful for realistic video generation. However, the generated motion in the video is usually not semantically meaningful due to the difficulty of determining the direction and magnitude in the StyleGAN latent space. In this paper, we propose a framework to generate realistic videos by leveraging multimodal (sound-image-text) embedding space. As sound provides the temporal contexts of the scene, our framework learns to generate a video that is semantically consistent with sound. First, our sound inversion module maps the audio directly into the StyleGAN latent space. We then incorporate the CLIP-based multimodal embedding space to further provide the audio-visual relationships. Finally, the proposed frame generator learns to find the trajectory in the latent space which is coherent with the corresponding sound and generates a video in a hierarchical manner. We provide the new high-resolution landscape video dataset (audio-visual pair) for the sound-guided video generation task. The experiments show that our model outperforms the state-of-the-art methods in terms of video quality. We further show several applications including image and video editing to verify the effectiveness of our method.

==> egbib.tex <==
@inproceedings{wang2020g3an,
  title={G3AN: disentangling appearance and motion for video generation},
  author={Wang, Yaohui and Bilinski, Piotr and Bremond, Francois and Dantcheva, Antitza},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={5264--5273},
  year={2020}
}

@inproceedings{saito2017temporal,
  title={Temporal generative adversarial nets with singular value clipping},
  author={Saito, Masaki and Matsumoto, Eiichi and Saito, Shunta},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={2830--2839},
  year={2017}
}
@article{vondrick2016generating,
  title={Generating videos with scene dynamics},
  author={Vondrick, Carl and Pirsiavash, Hamed and Torralba, Antonio},
  journal={Advances in neural information processing systems},
  volume={29},
  pages={613--621},
  year={2016}
}

@inproceedings{nawhal2020generating,
  title={Generating videos of zero-shot compositions of actions and objects},
  author={Nawhal, Megha and Zhai, Mengyao and Lehrmann, Andreas and Sigal, Leonid and Mori, Greg},
  booktitle={European Conference on Computer Vision},
  pages={382--401},
  year={2020},
  organization={Springer}
}

@inproceedings{dorkenwald2021stochastic,
  title={Stochastic Image-to-Video Synthesis using cINNs},
  author={Dorkenwald, Michael and Milbich, Timo and Blattmann, Andreas and Rombach, Robin and Derpanis, Konstantinos G and Ommer, Bjorn},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={3742--3753},
  year={2021}
}

@inproceedings{logacheva2020deeplandscape,
  title={Deeplandscape: Adversarial modeling of landscape videos},
  author={Logacheva, Elizaveta and Suvorov, Roman and Khomenko, Oleg and Mashikhin, Anton and Lempitsky, Victor},
  booktitle={European Conference on Computer Vision},
  pages={256--272},
  year={2020},
  organization={Springer}
}

@inproceedings{chen2020optical,
  title={Optical flow distillation: Towards efficient and stable video style transfer},
  author={Chen, Xinghao and Zhang, Yiman and Wang, Yunhe and Shu, Han and Xu, Chunjing and Xu, Chang},
  booktitle={European Conference on Computer Vision},
  pages={614--630},
  year={2020},
  organization={Springer}
}

@inproceedings{blattmann2021understanding,
  title={Understanding Object Dynamics for Interactive Image-to-Video Synthesis},
  author={Blattmann, Andreas and Milbich, Timo and Dorkenwald, Michael and Ommer, Bjorn},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={5171--5181},
  year={2021}
}

@inproceedings{ardino2021click,
  title={Click to Move: Controlling Video Generation with Sparse Motion},
  author={Ardino, Pierfrancesco and De Nadai, Marco and Lepri, Bruno and Ricci, Elisa and Lathuili{\`e}re, St{\'e}phane},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={14749--14758},
  year={2021}
}

@article{wu2021n,
  title={N$\backslash$" UWA: Visual Synthesis Pre-training for Neural visUal World creAtion},
  author={Wu, Chenfei and Liang, Jian and Ji, Lei and Yang, Fan and Fang, Yuejian and Jiang, Daxin and Duan, Nan},
  journal={arXiv preprint arXiv:2111.12417},
  year={2021}
}

@inproceedings{ji2021audio,
  title={Audio-driven emotional video portraits},
  author={Ji, Xinya and Zhou, Hang and Wang, Kaisiyuan and Wu, Wayne and Loy, Chen Change and Cao, Xun and Xu, Feng},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={14080--14089},
  year={2021}
}
@inproceedings{lahiri2021lipsync3d,
  title={LipSync3D: Data-Efficient Learning of Personalized 3D Talking Faces from Video using Pose and Lighting Normalization},
  author={Lahiri, Avisek and Kwatra, Vivek and Frueh, Christian and Lewis, John and Bregler, Chris},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={2755--2764},
  year={2021}
}

@article{le2021ccvs,
  title={CCVS: Context-aware Controllable Video Synthesis},
  author={Le Moing, Guillaume and Ponce, Jean and Schmid, Cordelia},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  year={2021}
}

@inproceedings{chatterjee2020sound2sight,
  title={Sound2Sight: Generating Visual Dynamics from Sound and Context},
  author={Chatterjee, Moitreya and Cherian, Anoop},
  booktitle={European Conference on Computer Vision},
  pages={701--719},
  year={2020},
  organization={Springer}
}

@inproceedings{tulyakov2018mocogan,
  title={Mocogan: Decomposing motion and content for video generation},
  author={Tulyakov, Sergey and Liu, Ming-Yu and Yang, Xiaodong and Kautz, Jan},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1526--1535},
  year={2018}
}
@inproceedings{hyun2021self,
  title={Self-Supervised Video GANs: Learning for Appearance Consistency and Motion Coherency},
  author={Hyun, Sangeek and Kim, Jihwan and Heo, Jae-Pil},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={10826--10835},
  year={2021}
}

@article{akbari2021vatt,
  title={Vatt: Transformers for multimodal self-supervised learning from raw video, audio and text},
  author={Akbari, Hassan and Yuan, Linagzhe and Qian, Rui and Chuang, Wei-Hong and Chang, Shih-Fu and Cui, Yin and Gong, Boqing},
  journal={arXiv preprint arXiv:2104.11178},
  year={2021}
}

@inproceedings{zolfaghari2021crossclr,
  title={CrossCLR: Cross-modal Contrastive Learning For Multi-modal Video Representations},
  author={Zolfaghari, Mohammadreza and Zhu, Yi and Gehler, Peter and Brox, Thomas},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={1450--1459},
  year={2021}
}

@inproceedings{
tian2021a,
title={A Good Image Generator Is What You Need for High-Resolution Video Synthesis},
author={Yu Tian and Jian Ren and Menglei Chai and Kyle Olszewski and Xi Peng and Dimitris N. Metaxas and Sergey Tulyakov},
booktitle={International Conference on Learning Representations},
year={2021},
url={https://openreview.net/forum?id=6puCSjH3hwA}
}

@article{skorokhodov2021stylegan,
  title={StyleGAN-V: A Continuous Video Generator with the Price, Image Quality and Perks of StyleGAN2},
  author={Skorokhodov, Ivan and Tulyakov, Sergey and Elhoseiny, Mohamed},
  journal={arXiv preprint arXiv:2112.14683},
  year={2021}
}

@article{gatys2016neural,
  title={A Neural Algorithm of Artistic Style},
  author={Gatys, Leon and Ecker, Alexander and Bethge, Matthias},
  journal={Journal of Vision},
  volume={16},
  number={12},
  pages={326--326},
  year={2016},
  publisher={The Association for Research in Vision and Ophthalmology}
}
@inproceedings{gatys2016image,
  title={Image style transfer using convolutional neural networks},
  author={Gatys, Leon A and Ecker, Alexander S and Bethge, Matthias},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={2414--2423},
  year={2016}
}
@InProceedings{Patashnik_2021_ICCV,
    author    = {Patashnik, Or and Wu, Zongze and Shechtman, Eli and Cohen-Or, Daniel and Lischinski, Dani},
    title     = {StyleCLIP: Text-Driven Manipulation of StyleGAN Imagery},
    booktitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)},
    month     = {October},
    year      = {2021},
    pages     = {2085-2094}
}
@incollection{fellbaum2010wordnet,
  title={WordNet},
  author={Fellbaum, Christiane},
  booktitle={Theory and applications of ontology: computer applications},
  pages={231--243},
  year={2010},
  publisher={Springer}
}
@inproceedings{harkonen2020ganspace,
  title={GANSpace: Discovering Interpretable GAN controls},
  author={H{\"a}rk{\"o}nen, Erik and Hertzman, Aaron and Lehtinen, Jaakko and Paris, Sylvain},
  booktitle={IEEE Conference on Neural Information Processing Systems;},
  year={2020}
}
@inproceedings{shen2021closed,
  title={Closed-form factorization of latent semantics in gans},
  author={Shen, Yujun and Zhou, Bolei},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={1532--1540},
  year={2021}
}
@article{radford2learning,
  title={Learning Transferable Visual Models From Natural Language Supervision},
  author={Radford, Alec and Kim, Jong Wook and Hallacy, Chris and Ramesh, Aditya and Goh, Gabriel and Agarwal, Sandhini and Sastry, Girish and Askell, Amanda and Mishkin, Pamela and Clark, Jack and others},
  journal={Image},
  volume={2},
  pages={T2}
}

@article{nitzan2020face,
  title={Face identity disentanglement via latent space mapping},
  author={Nitzan, Yotam and Bermano, Amit and Li, Yangyan and Cohen-Or, Daniel},
  journal={ACM Transactions on Graphics (TOG)},
  volume={39},
  number={6},
  pages={1--14},
  year={2020},
  publisher={ACM New York, NY, USA}
}

@inproceedings{karras2019style,
  title={A style-based generator architecture for generative adversarial networks},
  author={Karras, Tero and Laine, Samuli and Aila, Timo},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={4401--4410},
  year={2019}
}

@inproceedings{richardson2021encoding,
  title={Encoding in style: a stylegan encoder for image-to-image translation},
  author={Richardson, Elad and Alaluf, Yuval and Patashnik, Or and Nitzan, Yotam and Azar, Yaniv and Shapiro, Stav and Cohen-Or, Daniel},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={2287--2296},
  year={2021}
}
@inproceedings{wu2021stylespace,
  title={Stylespace analysis: Disentangled controls for stylegan image generation},
  author={Wu, Zongze and Lischinski, Dani and Shechtman, Eli},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={12863--12872},
  year={2021}
}
@inproceedings{dong2017semantic,
  title={Semantic image synthesis via adversarial learning},
  author={Dong, Hao and Yu, Simiao and Wu, Chao and Guo, Yike},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={5706--5714},
  year={2017}
}

@inproceedings{li2020manigan,
  title={Manigan: Text-guided image manipulation},
  author={Li, Bowen and Qi, Xiaojuan and Lukasiewicz, Thomas and Torr, Philip HS},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={7880--7889},
  year={2020}
}
@inproceedings{xia2021tedigan,
  title={TediGAN: Text-Guided Diverse Face Image Generation and Manipulation},
  author={Xia, Weihao and Yang, Yujiu and Xue, Jing-Hao and Wu, Baoyuan},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={2256--2265},
  year={2021}
}

@inproceedings{lee2020crossing,
  title={Crossing You in Style: Cross-modal Style Transfer from Music to Visual Arts},
  author={Lee, Cheng-Che and Lin, Wan-Yi and Shih, Yen-Ting and Kuo, Pei-Yi and Su, Li},
  booktitle={Proceedings of the 28th ACM International Conference on Multimedia},
  pages={3219--3227},
  year={2020}
}

@article{jeong2021tr,
  title={Tr$\ddot{a}$umerAI: Dreaming Music with StyleGAN},
  author={Jeong, Dasaem and Doh, Seungheon and Kwon, Taegyun},
  journal={arXiv preprint arXiv:2102.04680},
  year={2021}
}

@inproceedings{brouwer2020audio,
  title={Audio-reactive latent interpolations with StyleGAN},
  author={Brouwer, H},
  booktitle={NeurIPS 2020 Workshop on Machine Learning for Creativity and Design},
  year={2020}
}

@inproceedings{chen2020vggsound,
  title={Vggsound: A large-scale audio-visual dataset},
  author={Chen, Honglie and Xie, Weidi and Vedaldi, Andrea and Zisserman, Andrew},
  booktitle={ICASSP 2020-2020 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={721--725},
  year={2020},
  organization={IEEE}
}

@inproceedings{piczak2015esc,
  title={ESC: Dataset for environmental sound classification},
  author={Piczak, Karol J},
  booktitle={Proceedings of the 23rd ACM international conference on Multimedia},
  pages={1015--1018},
  year={2015}
}

@inproceedings{Salamon:UrbanSound:ACMMM:14,
    Address = {Orlando, FL, USA},
    Author = {Salamon, J. and Jacoby, C. and Bello, J. P.},
    Booktitle = {22nd {ACM} International Conference on Multimedia (ACM-MM'14)},
    Month = {Nov.},
    Pages = {1041--1044},
    Title = {A Dataset and Taxonomy for Urban Sound Research},
    Year = {2014}
    
    
    
    }
@article{goodfellow2014generative,
  title={Generative adversarial nets},
  author={Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  journal={Advances in neural information processing systems},
  volume={27},
  year={2014}
}
    


@inproceedings{hershey2017cnn,
  title={CNN architectures for large-scale audio classification},
  author={Hershey, Shawn and Chaudhuri, Sourish and Ellis, Daniel PW and Gemmeke, Jort F and Jansen, Aren and Moore, R Channing and Plakal, Manoj and Platt, Devin and Saurous, Rif A and Seybold, Bryan and others},
  booktitle={2017 ieee international conference on acoustics, speech and signal processing (icassp)},
  pages={131--135},
  year={2017},
  organization={IEEE}
}
@article{yu2015lsun,
  title={LSUN: Construction of a Large-scale Image Dataset using Deep Learning with Humans in the Loop},
  author={Yu, Fisher and Zhang, Yinda and Song, Shuran and Seff, Ari and Xiao, Jianxiong},
  publisher={Citeseer},
   year={2015}
}
@inproceedings{voynov2020unsupervised,
  title={Unsupervised discovery of interpretable directions in the gan latent space},
  author={Voynov, Andrey and Babenko, Artem},
  booktitle={International Conference on Machine Learning},
  pages={9786--9796},
  year={2020},
  organization={PMLR}
}

@article{xia2021gan,
  title={Gan inversion: A survey},
  author={Xia, Weihao and Zhang, Yulun and Yang, Yujiu and Xue, Jing-Hao and Zhou, Bolei and Yang, Ming-Hsuan},
  journal={arXiv preprint arXiv:2101.05278},
  year={2021}
}

@article{oord2016wavenet,
  title={Wavenet: A generative model for raw audio},
  author={Oord, Aaron van den and Dieleman, Sander and Zen, Heiga and Simonyan, Karen and Vinyals, Oriol and Graves, Alex and Kalchbrenner, Nal and Senior, Andrew and Kavukcuoglu, Koray},
  journal={arXiv preprint arXiv:1609.03499},
  year={2016}
}
@inproceedings{wan2019towards,
  title={Towards audio to scene image synthesis using generative adversarial network},
  author={Wan, Chia-Hung and Chuang, Shun-Po and Lee, Hung-Yi},
  booktitle={ICASSP 2019-2019 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={496--500},
  year={2019},
  organization={IEEE}
}
@inproceedings{hao2018cmcgan,
  title={Cmcgan: A uniform framework for cross-modal visual-audio mutual generation},
  author={Hao, Wangli and Zhang, Zhaoxiang and Guan, He},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={32},
  number={1},
  year={2018}
}

@article{zhu2021deep,
  title={Deep audio-visual learning: A survey},
  author={Zhu, Hao and Luo, Man-Di and Wang, Rui and Zheng, Ai-Hua and He, Ran},
  journal={International Journal of Automation and Computing},
  pages={1--26},
  year={2021},
  publisher={Springer}
}

@inproceedings{qiu2018image,
  title={Image generation associated with music data},
  author={Qiu, Yue and Kataoka, Hirokatsu},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition Workshops},
  pages={2510--2513},
  year={2018}
}

@inproceedings{oh2019speech2face,
  title={Speech2face: Learning the face behind a voice},
  author={Oh, Tae-Hyun and Dekel, Tali and Kim, Changil and Mosseri, Inbar and Freeman, William T and Rubinstein, Michael and Matusik, Wojciech},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={7539--7548},
  year={2019}
}

@inproceedings{nagrani2018learnable,
  title={Learnable pins: Cross-modal embeddings for person identity},
  author={Nagrani, Arsha and Albanie, Samuel and Zisserman, Andrew},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={71--88},
  year={2018}
}

@article{DBLP:journals/corr/AytarVT17,
  author    = {Yusuf Aytar and
               Carl Vondrick and
               Antonio Torralba},
  title     = {See, Hear, and Read: Deep Aligned Representations},
  journal   = {CoRR},
  volume    = {abs/1706.00932},
  year      = {2017},
  url       = {http://arxiv.org/abs/1706.00932},
  eprinttype = {arXiv},
  eprint    = {1706.00932},
  timestamp = {Mon, 13 Aug 2018 16:48:33 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/AytarVT17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{chen2021distilling,
  title={Distilling Audio-Visual Knowledge by Compositional Contrastive Learning},
  author={Chen, Yanbei and Xian, Yongqin and Koepke, A and Shan, Ying and Akata, Zeynep},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={7016--7025},
  year={2021}
}
@inproceedings{mazumder2021avgzslnet,
  title={Avgzslnet: Audio-visual generalized zero-shot learning by reconstructing label features from multi-modal embeddings},
  author={Mazumder, Pratik and Singh, Pravendra and Parida, Kranti Kumar and Namboodiri, Vinay P},
  booktitle={Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision},
  pages={3090--3099},
  year={2021}
}

@inproceedings{sun2020learning,
  title={Learning relationships between text, audio, and video via deep canonical correlation for multimodal language analysis},
  author={Sun, Zhongkai and Sarma, Prathusha and Sethares, William and Liang, Yingyu},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={34},
  number={05},
  pages={8992--8999},
  year={2020}
}

@inproceedings{park19e_interspeech,
  author={Daniel S. Park and William Chan and Yu Zhang and Chung-Cheng Chiu and Barret Zoph and Ekin D. Cubuk and Quoc V. Le},
  title={{SpecAugment: A Simple Data Augmentation Method for Automatic Speech Recognition}},
  year=2019,
  booktitle={Proc. Interspeech 2019},
  pages={2613–2617},
  doi={10.21437/Interspeech.2019-2680}
}

@incollection{golub1971singular,
  title={Singular value decomposition and least squares solutions},
  author={Golub, Gene H and Reinsch, Christian},
  booktitle={Linear algebra},
  pages={134--151},
  year={1971},
  publisher={Springer}
}

@article{kay2017kinetics,
  title={The kinetics human action video dataset},
  author={Kay, Will and Carreira, Joao and Simonyan, Karen and Zhang, Brian and Hillier, Chloe and Vijayanarasimhan, Sudheendra and Viola, Fabio and Green, Tim and Back, Trevor and Natsev, Paul and others},
  journal={arXiv preprint arXiv:1705.06950},
  year={2017}
}
@misc{gatys2015neural,
      title={A Neural Algorithm of Artistic Style}, 
      author={Leon A. Gatys and Alexander S. Ecker and Matthias Bethge},
      year={2015},
      eprint={1508.06576},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}
@article{soomro2012ucf101,
  title={UCF101: A dataset of 101 human actions classes from videos in the wild},
  author={Soomro, Khurram and Zamir, Amir Roshan and Shah, Mubarak},
  journal={arXiv preprint arXiv:1212.0402},
  year={2012}
}

@inproceedings{caba2015activitynet,
  title={Activitynet: A large-scale video benchmark for human activity understanding},
  author={Caba Heilbron, Fabian and Escorcia, Victor and Ghanem, Bernard and Carlos Niebles, Juan},
  booktitle={Proceedings of the ieee conference on computer vision and pattern recognition},
  pages={961--970},
  year={2015}
}


@article{alayrac2020self,
  title={Self-Supervised MultiModal Versatile Networks.},
  author={Alayrac, Jean-Baptiste and Recasens, Adria and Schneider, Rosalia and Arandjelovic, Relja and Ramapuram, Jason and De Fauw, Jeffrey and Smaira, Lucas and Dieleman, Sander and Zisserman, Andrew},
  journal={NeurIPS},
  volume={2},
  number={6},
  pages={7},
  year={2020}
}

@inproceedings{deng2019arcface,
  title={Arcface: Additive angular margin loss for deep face recognition},
  author={Deng, Jiankang and Guo, Jia and Xue, Niannan and Zafeiriou, Stefanos},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={4690--4699},
  year={2019}
}
@article{saleh2016large,
  title={Large-scale Classification of Fine-Art Paintings: Learning The Right Metric on The Right Feature},
  author={Saleh, Babak and Elgammal, Ahmed},
  journal={International Journal for Digital Art History},
  number={2},
  year={2016}
}
@inproceedings{jiang2021language,
  title={Language-Guided Global Image Editing via Cross-Modal Cyclic Mechanism},
  author={Jiang, Wentao and Xu, Ning and Wang, Jiayun and Gao, Chen and Shi, Jing and Lin, Zhe and Liu, Si},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={2115--2124},
  year={2021}
}
@inproceedings{nam2018tagan,
  title={Text-Adaptive Generative Adversarial Networks: Manipulating Images with Natural Language},
  author={Nam, Seonghyeon and Kim, Yunji and Kim, Seon Joo},
  booktitle={Advances in Neural Information Processing Systems (NeurIPS)},
  year={2018}
}

@inproceedings{el2019tell,
  title={Tell, draw, and repeat: Generating and modifying images based on continual linguistic instruction},
  author={El-Nouby, Alaaeldin and Sharma, Shikhar and Schulz, Hannes and Hjelm, Devon and Asri, Layla El and Kahou, Samira Ebrahimi and Bengio, Yoshua and Taylor, Graham W},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={10304--10312},
  year={2019}
}
@inproceedings{park2019semantic,
  title={Semantic image synthesis with spatially-adaptive normalization},
  author={Park, Taesung and Liu, Ming-Yu and Wang, Ting-Chun and Zhu, Jun-Yan},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={2337--2346},
  year={2019}
}
@inproceedings{
dosovitskiy2021an,
title={An Image is Worth 16x16 Words: Transformers for Image Recognition at Scale},
author={Alexey Dosovitskiy and Lucas Beyer and Alexander Kolesnikov and Dirk Weissenborn and Xiaohua Zhai and Thomas Unterthiner and Mostafa Dehghani and Matthias Minderer and Georg Heigold and Sylvain Gelly and Jakob Uszkoreit and Neil Houlsby},
booktitle={International Conference on Learning Representations},
year={2021},
url={https://openreview.net/forum?id=YicbFdNTTy}
}
@article{radford2019language,
  title={Language models are unsupervised multitask learners},
  author={Radford, Alec and Wu, Jeffrey and Child, Rewon and Luan, David and Amodei, Dario and Sutskever, Ilya and others},
  journal={OpenAI blog},
  volume={1},
  number={8},
  pages={9},
  year={2019}
}


@article{10.1145/3450626.3459838,
author = {Tov, Omer and Alaluf, Yuval and Nitzan, Yotam and Patashnik, Or and Cohen-Or, Daniel},
title = {Designing an Encoder for StyleGAN Image Manipulation},
year = {2021},
issue_date = {August 2021},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {40},
number = {4},
issn = {0730-0301},
url = {https://doi.org/10.1145/3450626.3459838},
doi = {10.1145/3450626.3459838},
journal = {ACM Trans. Graph.},
month = {jul},
articleno = {133},
numpages = {14},
keywords = {image editing, latent space, generative adversarial networks}
}


@inproceedings{abdal2019image2stylegan,
  title={Image2stylegan: How to embed images into the stylegan latent space?},
  author={Abdal, Rameen and Qin, Yipeng and Wonka, Peter},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={4432--4441},
  year={2019}
}

@inproceedings{karras2020analyzing,
  title={Analyzing and improving the image quality of stylegan},
  author={Karras, Tero and Laine, Samuli and Aittala, Miika and Hellsten, Janne and Lehtinen, Jaakko and Aila, Timo},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={8110--8119},
  year={2020}
}

@inproceedings{smith2017cyclical,
  title={Cyclical learning rates for training neural networks},
  author={Smith, Leslie N},
  booktitle={2017 IEEE winter conference on applications of computer vision (WACV)},
  pages={464--472},
  year={2017},
  organization={IEEE}
}

@inproceedings{choi2018stargan,
author={Yunjey Choi and Minje Choi and Munyoung Kim and Jung-Woo Ha and Sunghun Kim and Jaegul Choo},
title={StarGAN: Unified Generative Adversarial Networks for Multi-Domain Image-to-Image Translation},
booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
year={2018}
}

@inproceedings{philion2020learning,
  title={Learning to evaluate perception models using planner-centric metrics},
  author={Philion, Jonah and Kar, Amlan and Fidler, Sanja},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={14055--14064},
  year={2020}
}

@inproceedings{altwaijry2016learning,
  title={Learning to match aerial images with deep attentive architectures},
  author={Altwaijry, Hani and Trulls, Eduard and Hays, James and Fua, Pascal and Belongie, Serge},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={3539--3547},
  year={2016}
}

@inproceedings{zhou2018interpretable,
  title={Interpretable basis decomposition for visual explanation},
  author={Zhou, Bolei and Sun, Yiyou and Bau, David and Torralba, Antonio},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={119--134},
  year={2018}
}

@inproceedings{shaham2019singan,
  title={Singan: Learning a generative model from a single natural image},
  author={Shaham, Tamar Rott and Dekel, Tali and Michaeli, Tomer},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={4570--4580},
  year={2019}
}

@ARTICLE{9524590,
  author={Mesaros, Annamaria and Heittola, Toni and Virtanen, Tuomas and Plumbley, Mark D.},
  journal={IEEE Signal Processing Magazine}, 
  title={Sound Event Detection: A tutorial}, 
  year={2021},
  volume={38},
  number={5},
  pages={67-83},
  doi={10.1109/MSP.2021.3090678}}
  
 @misc{wu2021wav2clip,
      title={Wav2CLIP: Learning Robust Audio Representations From CLIP}, 
      author={Ho-Hsiang Wu and Prem Seetharaman and Kundan Kumar and Juan Pablo Bello},
      year={2021},
      eprint={2110.11499},
      archivePrefix={arXiv},
      primaryClass={cs.SD}
}

@misc{guzhov2021audioclip,
      title={AudioCLIP: Extending CLIP to Image, Text and Audio}, 
      author={Andrey Guzhov and Federico Raue and Jörn Hees and Andreas Dengel},
      year={2021},
      eprint={2106.13043},
      archivePrefix={arXiv},
      primaryClass={cs.SD}
}

@article{guzhov2021esresne,
  title={ESResNe (X) t-fbsp: Learning Robust Time-Frequency Transformation of Audio},
  author={Guzhov, Andrey and Raue, Federico and Hees, J{\"o}rn and Dengel, Andreas},
  journal={arXiv preprint arXiv:2104.11587},
  year={2021}
}
@article{oord2018representation,
  title={Representation learning with contrastive predictive coding},
  author={Oord, Aaron van den and Li, Yazhe and Vinyals, Oriol},
  journal={arXiv preprint arXiv:1807.03748},
  year={2018}
}
@article{van2008visualizing,
  title={Visualizing High-Dimensional Data Using t-629 SNE},
  author={van der Maaten, LJP and Hinton, GE},
  journal={Journal of Machine Learning Research},
  volume={9},
  number={2579-2605},
  pages={630},
  year={2008}
}

@article{zhang2020contrastive,
  title={Contrastive learning of medical visual representations from paired images and text},
  author={Zhang, Yuhao and Jiang, Hang and Miura, Yasuhide and Manning, Christopher D and Langlotz, Curtis P},
  journal={arXiv preprint arXiv:2010.00747},
  year={2020}
}



@inproceedings{Johnson2016Perceptual,
  title={Perceptual losses for real-time style transfer and super-resolution},
  author={Johnson, Justin and Alahi, Alexandre and Fei-Fei, Li},
  booktitle={European Conference on Computer Vision},
  year={2016}
}

@inproceedings{zhang2018perceptual,
  title={The Unreasonable Effectiveness of Deep Features as a Perceptual Metric},
  author={Zhang, Richard and Isola, Phillip and Efros, Alexei A and Shechtman, Eli and Wang, Oliver},
  booktitle={CVPR},
  year={2018}
}

@InProceedings{Skorokhodov_2021_ICCV,
    author    = {Skorokhodov, Ivan and Sotnikov, Grigorii and Elhoseiny, Mohamed},
    title     = {Aligning Latent and Image Spaces To Connect the Unconnectable},
    booktitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)},
    month     = {October},
    year      = {2021},
    pages     = {14144-14153}
}

@inproceedings{suris2018cross,
  title={Cross-modal embeddings for video and audio retrieval},
  author={Sur{\’\i}s, Didac and Duarte, Amanda and Salvador, Amaia and Torres, Jordi and Gir{\’o}-i-Nieto, Xavier},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV) Workshops},
  pages={0--0},
  year={2018}
}

@article{chu2020learning,
  title={Learning temporal coherence via self-supervision for GAN-based video generation},
  author={Chu, Mengyu and Xie, You and Mayer, Jonas and Leal-Taix{\'e}, Laura and Thuerey, Nils},
  journal={ACM Transactions on Graphics (TOG)},
  volume={39},
  number={4},
  pages={75--1},
  year={2020},
  publisher={ACM New York, NY, USA}
}

@article{karras2021alias,
  title={Alias-free generative adversarial networks},
  author={Karras, Tero and Aittala, Miika and Laine, Samuli and H{\"a}rk{\"o}nen, Erik and Hellsten, Janne and Lehtinen, Jaakko and Aila, Timo},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  year={2021}
}
@article{kingma2013auto,
  title={Auto-encoding variational bayes},
  author={Kingma, Diederik P and Welling, Max},
  journal={arXiv preprint arXiv:1312.6114},
  year={2013}
}

@article{fox2021stylevideogan,
  title={Stylevideogan: A temporal generative model using a pretrained stylegan},
  author={Fox, Gereon and Tewari, Ayush and Elgharib, Mohamed and Theobalt, Christian},
  journal={arXiv preprint arXiv:2107.07224},
  year={2021}
}
@article{yan2021videogpt,
  title={Videogpt: Video generation using vq-vae and transformers},
  author={Yan, Wilson and Zhang, Yunzhi and Abbeel, Pieter and Srinivas, Aravind},
  journal={arXiv preprint arXiv:2104.10157},
  year={2021}
}

@inproceedings{kurmi2021collaborative,
  title={Collaborative learning to generate audio-video jointly},
  author={Kurmi, Vinod K and Bajaj, Vipul and Patro, Badri N and Venkatesh, KS and Namboodiri, Vinay P and Jyothi, Preethi},
  booktitle={ICASSP 2021-2021 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={4180--4184},
  year={2021},
  organization={IEEE}
}
@inproceedings{duan2021cascade,
  title={Cascade attention guided residue learning gan for cross-modal translation},
  author={Duan, Bin and Wang, Wei and Tang, Hao and Latapie, Hugo and Yan, Yan},
  booktitle={2020 25th International Conference on Pattern Recognition (ICPR)},
  pages={1336--1343},
  year={2021},
  organization={IEEE}
}
@article{lee2021sound,
  title={Sound-Guided Semantic Image Manipulation},
  author={Lee, Seung Hyun and Roh, Wonseok and Byeon, Wonmin and Yoon, Sang Ho and Kim, Chan Young and Kim, Jinkyu and Kim, Sangpil},
  journal={arXiv preprint arXiv:2112.00007},
  year={2021}
}

@inproceedings{hao2018cmcgan,
  title={Cmcgan: A uniform framework for cross-modal visual-audio mutual generation},
  author={Hao, Wangli and Zhang, Zhaoxiang and Guan, He},
  booktitle={Proceedings of the AAAI conference on artificial intelligence},
  volume={32},
  number={1},
  year={2018}
}
@article{li2018creating,
  title={Creating a multitrack classical music performance dataset for multimodal music analysis: Challenges, insights, and applications},
  author={Li, Bochen and Liu, Xinzhao and Dinesh, Karthik and Duan, Zhiyao and Sharma, Gaurav},
  journal={IEEE Transactions on Multimedia},
  volume={21},
  number={2},
  pages={522--535},
  year={2018},
  publisher={IEEE}
}

@article{pix2pix2017,
  title={Image-to-Image Translation with Conditional Adversarial Networks},
  author={Isola, Phillip and Zhu, Jun-Yan and Zhou, Tinghui and Efros, Alexei A},
  journal={CVPR},
  year={2017}
}

@InProceedings{He_2016_CVPR,
author = {He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
title = {Deep Residual Learning for Image Recognition},
booktitle = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2016}
}

@inproceedings{NIPS2017_3f5ee243,
 author = {Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, \L ukasz and Polosukhin, Illia},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {I. Guyon and U. V. Luxburg and S. Bengio and H. Wallach and R. Fergus and S. Vishwanathan and R. Garnett},
 pages = {},
 publisher = {Curran Associates, Inc.},
 title = {Attention is All you Need},
 url = {https://proceedings.neurips.cc/paper/2017/file/3f5ee243547dee91fbd053c1c4a845aa-Paper.pdf},
 volume = {30},
 year = {2017}
}

@InProceedings{NIPS2019_workshop,
author = {Han-Hung Lee, Da-Gin Wu, and Hwann-Tzong Chen},
title = {Stylizing Audio Reactive Visuals},
url = {https://neurips2019creativity.github.io/doc/Stylizing%20Audio%20Reactive%20Visuals.pdf},
year = {2019}
}

@inproceedings{chen2019hierarchical,
  title={Hierarchical cross-modal talking face generation with dynamic pixel-wise loss},
  author={Chen, Lele and Maddox, Ross K and Duan, Zhiyao and Xu, Chenliang},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={7832--7841},
  year={2019}
}

@inproceedings{Das2020SpeechDrivenFA,
  title={Speech-Driven Facial Animation Using Cascaded GANs for Learning of Motion and Texture},
  author={Dipanjan Das and S. Biswas and Sanjana Sinha and Brojeshwar Bhowmick},
  booktitle={ECCV},
  year={2020}
}

@article{Suwajanakorn2017SynthesizingO,
  title={Synthesizing Obama},
  author={Supasorn Suwajanakorn and Steven M. Seitz and Ira Kemelmacher-Shlizerman},
  journal={ACM Transactions on Graphics (TOG)},
  year={2017},
  volume={36},
  pages={1 - 13}
}

@inproceedings{Chen2020TalkingheadGW,
  title={Talking-head Generation with Rhythmic Head Motion},
  author={Lele Chen and Guofeng Cui and Celong Liu and Zhong Li and Ziyi Kou and Yi Xu and Chenliang Xu},
  booktitle={ECCV},
  year={2020}
}

@InProceedings{Richard_2021_WACV,
    author    = {Richard, Alexander and Lea, Colin and Ma, Shugao and Gall, Jurgen and de la Torre, Fernando and Sheikh, Yaser},
    title     = {Audio- and Gaze-Driven Facial Animation of Codec Avatars},
    booktitle = {Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision (WACV)},
    month     = {January},
    year      = {2021},
    pages     = {41-50}
}

@inproceedings{Thies2020NeuralVP,
  title={Neural Voice Puppetry: Audio-driven Facial Reenactment},
  author={Justus Thies and Mohamed A. Elgharib and Ayush Tewari and Christian Theobalt and Matthias Nie{\ss}ner},
  booktitle={ECCV},
  year={2020}
}

@inproceedings{wang2021facevid2vid,
   author    = {Ting-Chun Wang and Arun Mallya and Ming-Yu Liu},
   title     = {One-Shot Free-View Neural Talking-Head Synthesis for Video Conferencing},
   booktitle = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
   year      = {2021},
}

@inproceedings{wu2021imitating,
  title={Imitating Arbitrary Talking Style for Realistic Audio-Driven Talking Face Synthesis},
  author={Wu, Haozhe and Jia, Jia and Wang, Haoyu and Dou, Yishun and Duan, Chao and Deng, Qingshan},
  booktitle={Proceedings of the 29th ACM International Conference on Multimedia},
  pages={1478--1486},
  year={2021}
}

@misc{yi2020audiodriven,
      title={Audio-driven Talking Face Video Generation with Learning-based Personalized Head Pose}, 
      author={Ran Yi and Zipeng Ye and Juyong Zhang and Hujun Bao and Yong-Jin Liu},
      year={2020},
      eprint={2002.10137},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@article{Yang:2020:MakeItTalk,
	Author    = {Yang Zhou and Xintong Han and Eli Shechtman and Jose Echevarria and Evangelos Kalogerakis and Dingzeyu Li},
	Title     = {MakeItTalk: Speaker-Aware Talking-Head Animation},
	Journal   = {ACM Transactions on Graphics},
	Volume    = {39},
	Number    = {6},
	Year      = {2020},
}

@article{unterthiner2018towards,
  title={Towards accurate generative models of video: A new metric \& challenges},
  author={Unterthiner, Thomas and van Steenkiste, Sjoerd and Kurach, Karol and Marinier, Raphael and Michalski, Marcin and Gelly, Sylvain},
  journal={arXiv preprint arXiv:1812.01717},
  year={2018}
}

@InProceedings{Kuehne11,
   author= "Kuehne, H. and Jhuang, H. and Garrote, E. and Poggio, T. and Serre, T.",
   title = "{HMDB}: a large video database for human motion recognition",
   booktitle = "Proceedings of the International Conference on Computer Vision (ICCV)",
   year = "2011",
}

@inproceedings{carreira2017quo,
  title={Quo vadis, action recognition? a new model and the kinetics dataset},
  author={Carreira, Joao and Zisserman, Andrew},
  booktitle={proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={6299--6308},
  year={2017}
}

@article{salimans2016improved,
  title={Improved techniques for training gans},
  author={Salimans, Tim and Goodfellow, Ian and Zaremba, Wojciech and Cheung, Vicki and Radford, Alec and Chen, Xi},
  journal={Advances in neural information processing systems},
  volume={29},
  year={2016}
}

@article{Chung2014EmpiricalEO,
  title={Empirical Evaluation of Gated Recurrent Neural Networks on Sequence Modeling},
  author={Junyoung Chung and Çaglar G{\"u}lçehre and Kyunghyun Cho and Yoshua Bengio},
  journal={ArXiv},
  year={2014},
  volume={abs/1412.3555}
}

@inproceedings{szegedy2016rethinking,
  title={Rethinking the inception architecture for computer vision},
  author={Szegedy, Christian and Vanhoucke, Vincent and Ioffe, Sergey and Shlens, Jon and Wojna, Zbigniew},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition },
  pages={2818--2826},
  year={2016}
}

@article{unterthiner2019fvd,
  title={FVD: A new metric for video generation},
  author={Unterthiner, Thomas and van Steenkiste, Sjoerd and Kurach, Karol and Marinier, Rapha{\"e}l and Michalski, Marcin and Gelly, Sylvain},
  year={2019}
}


@INPROCEEDINGS{5206848,
  author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Kai Li and Li Fei-Fei},
  booktitle={2009 IEEE Conference on Computer Vision and Pattern Recognition}, 
  title={ImageNet: A large-scale hierarchical image database}, 
  year={2009},
  volume={},
  number={},
  pages={248-255},
  doi={10.1109/CVPR.2009.5206848}}
  
@ARTICLE{1163420,
  author={Davis, S. and Mermelstein, P.},
  journal={IEEE Transactions on Acoustics, Speech, and Signal Processing}, 
  title={Comparison of parametric representations for monosyllabic word recognition in continuously spoken sentences}, 
  year={1980},
  volume={28},
  number={4},
  pages={357-366},
  doi={10.1109/TASSP.1980.1163420}}
  
@article{DBLP:journals/corr/UlyanovVL16,
  author    = {Dmitry Ulyanov and
               Andrea Vedaldi and
               Victor S. Lempitsky},
  title     = {Instance Normalization: The Missing Ingredient for Fast Stylization},
  journal   = {CoRR},
  volume    = {abs/1607.08022},
  year      = {2016},
  url       = {http://arxiv.org/abs/1607.08022},
  eprinttype = {arXiv},
  eprint    = {1607.08022},
  timestamp = {Mon, 13 Aug 2018 16:47:58 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/UlyanovVL16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Maaten2008VisualizingDU,
  title={Visualizing Data using t-SNE},
  author={Laurens van der Maaten and Geoffrey E. Hinton},
  journal={Journal of Machine Learning Research},
  year={2008},
  volume={9},
  pages={2579-2605}
}

==> tex/need-to-use.tex <==
% There are three major differences between ours and the existing  video generation method. \textbf{(1)} Sound is used as a constraint. Unlike the existing StyleGAN inversion method~\cite{xia2021tedigan}, it takes sound as input, not image modal. To find the directions that correspond to the input sound, the sound latent code ${\bf {w}}_a \in \mathcal{W}+$ is mixed with the randomly sampled latent code ${\bf w}\in \mathcal{W}+$ then projected to the latent space. After that, we extend this to a time sequence for sound-guided video generation. We select the specific layer of the latent code of time step $t-1$ and the specific layer of the sound inverted latent code to obtain the latent code of time step $t$ with the next sound as constraints. \textbf{(2)} Our method automatically learns the hierarchical style changes. We use three separate recurrent StyleGAN~\cite{karras2019style} generator blocks (course, mid, fine) to predict various levels of motion details. \textbf{(3)} it uses CLIP~\cite{radford2learning}'s prior knowledge to maintain semantic consistency between sound and generated image. We extend Section 3.1 over time T frame to create a video. Sound-guided video of $T$ frames is represented by a sequence of length $T$ in the $\mathcal{W}+$ space $[G({\bf{\hat{w}}}_a^1), G({\bf{\hat{w}}}_a^2),...,G({\bf{\hat{w}}}_a^T)]$. The sound-guided video generation process is shown in Fig.~\ref{fig:overview}. We split the input sound into fixed-length segments. Each segment is used to guide the motion trajectory in the latent space at each time step. Our sound-guided frame generator learns to predict the next direction and magnitude of the movement from the current point in the latent space. After that, like MocoGAN-HD~\cite{tian2021a}, 3D-discriminator and 2D-discriminator determine whether the generated video is a synthesized video or real video.



% \begin{table}
%     %\vspace{-2em}
%     \begin{center}
%     \caption{High Fidelity Audio-visual Landscape Video Dataset Class Information.}
%     %\vspace{-2em}
%     \label{table:landscape-dataset}
%     \resizebox{\textwidth}{!}{% 
%         \begin{tabular}{lcccccccccc}\toprule
%         %\hline\noalign{\smallskip}
%         Class & Thunderstorm & Waterfall & Volcano & Squishing Water & Wind & Fire & Raining & Underwater & Splashing Water & Total \\\midrule
%         %\noalign{\smallskip}\hline\noalign{\smallskip}
%         \#Video & 280 & 270 & 60 & 1610 & 1835 & 1365 & 1825 & 260 & 1775 & 9280 \\\bottomrule
%     %\hline
%     \end{tabular}}
%     \end{center}
%     %\vspace{-3.5em}
% \end{table}



\myparagraph{Was in Section 3.2}
Our solution to invert the sound for video generation is to train jointly an sound inversion module $E_a(\cdot) :\mathcal{X}_a\rightarrow\mathcal{Z}$ and recurrent blocks $E_\text{RNN}(\cdot)$. In our training process, the latent code ${\bf {w}}_0$ is randomly sampled. At time step $t$, the network outputs the latent code $\hat{\bf {w}}^t_a \in \mathcal{W}+$ from the given real audio ${\bf{x}}^t_a$. The next frame $\hat{\bf{x}}_v^{t+1}$ generated from the previous frame can be formulated as follows
\begin{equation}
\hat{\bf{x}}_v^{t+1} = G(E_a({\bf{x}}_a^t)+{\bf{w}}^t),
\label{loss:psp}
\end{equation}

% The learnable parameters of encoder $E_a$ is optimized by minimizing the pixel-wise $\mathcal{L}_2$ loss between ${\bf{x}}_v^{t+1}$ and $\tilde{\bf{x}}_v^{t+1}$ with
% \begin{equation}
% \text{min}_{\theta_{E_a}}{\mathcal{L}_{2}^{t+1}}=||{\bf{x}}_v^{t+1} - {\tilde{\bf{x}}}_v^{t+1} ||^{2}_{2},
% \label{loss:image_inversion}
% \end{equation}

% where $\theta_E$ denotes the learnable parameter of the audio encoder $E_a(\cdot)$. In particular, Ricahrdson, \textit{et al}.~\cite{richardson2021encoding} use perceptual loss~\cite{Johnson2016Perceptual} and LPIPS~\cite{zhang2018perceptual} as image generation loss for stronger supervision, which preserves better image quality compared to the standard perceptual loss. The perceptual loss ${\mathcal{L}_{\text{LPIPS}}}$ is formulated as follows 
% \begin{equation}
% \text{min}_{\theta_{E_a}}{\mathcal{L}_{\text{LPIPS}}^{t+1}}=||F({\bf{x}}_v^{t+1})-F({\tilde{\bf{x}}}_v^{t+1}))||^2_{2}.
% \label{loss:image_inversion_up}
% \end{equation}

The inversion module $E_a(\cdot)$ predicts input real audio ${\bf{x}}_a$ as a latent code. We further define the regularization loss function so that the generated output image is close to the generation output of the mean latent vector:
\begin{equation}
\underset{\theta_{E_a}}{\text{min}}\,{\mathcal{L}_{\text{reg}}^{t+1}}=||E_a({\bf{x}}_a^t) -{\bar{\bf{w}}}||^{2}_{2}.
\label{loss:image_inversion_reg}
\end{equation}

We minimize the cosine distance between the audio input ${\bf{x}}_a^t$ and the CLIP embedding vector of the reconstructed image $\tilde{\bf{x}}_v^t$, which is shown useful to improve the quality of the latent representation
\begin{equation}
    \underset{\theta_{E_a}}{\text{min}}\,{\mathcal{L}_{\text{CLIP}}^{(a \leftrightarrow v) t+1}} = 1 - {F_v(\tilde{\bf{x}}_v^{t+1})\cdot F_a({\bf{x}}_a^{t}) \over ||F_v(\tilde{\bf{x}}_v^{t+1})|| \cdot ||F_a({\bf{x}}_a^{t})||},
    \label{loss:image_inversion_clip}
\end{equation}

% where $d_{cos}({\bf{x}}_a^t, \tilde{\bf{x}}_v^{t+1})$ denotes the cosine distance between the normalized CLIP image embedding of $\tilde{\bf{x}}^{t+1}_v$ and the normalized CLIP sound embedding of ${\bf{x}}^{t+1}_a$. 
where $F_v(\cdot)$ and $F_a(\cdot)$ are CLIP's image encoder and sound encoder. Formally, our total loss at the time step $t$ is a weighted combination of these loss functions~(Eq.~\ref{loss:image_inversion_reg} and Eq.~\ref{loss:image_inversion_clip}) as follows:
\begin{equation}
    \underset{\theta_{E_a}}{\text{min}}\,{\mathcal{L}_{total}} ={1 \over T}\sum_{t=0}^{T-1}{(\lambda_{1}\mathcal{L}^{t+1}_{reg} + \lambda_{2}\mathcal{L}^{(a \leftrightarrow v)t+1}_\text{CLIP} + \lambda_{3}\mathcal{L}^{(t \leftrightarrow v)t+1}_\text{CLIP})}.
\end{equation}
$\lambda_1$, $\lambda_2$, $\lambda_3$ are the weights of the loss function. To improve the image quality, the sound-guided video generator minimizes the multi-modal cosine distance in Eq.~\ref{loss:image_inversion_clip}. We consider not only the cosine distance between image and sound embeddings, but also the cosine distance between image and text label embeddings. $T$ is the length of the video sequence, and the total loss is the average of the weighted loss for each time step. With the trained inversion module, we move the audio input to $\mathcal{W}+$ space and get the initial latent code for video generation.

Therefore, the total loss of the generator is:
\begin{equation}
    \mathcal{L}_G=-\text{log}D_V({\bf{v}}) -\text{log}D_I({\bf{v}}) +{1 \over T}\sum_{t=0}^{T-1}{(\lambda_{1}\mathcal{L}^{t+1}_{reg} + \lambda_{2}\mathcal{L}^{(a \leftrightarrow v)t+1}_\text{CLIP} + \lambda_{3}\mathcal{L}^{(t \leftrightarrow v)t+1}_\text{CLIP})}.
    \label{loss:total_loss}
\end{equation}
